Secure Multi-hop Telemetry Broadcasts for UAV Swarm Communication

Unmanned Aerial Vehicles (UAVs) are evolving as adaptable platforms for a wide range of applications such as precise inspections, emergency response, and remote sensing. Autonomous UAV swarms require efficient and stable communication during deployment for a successful mission execution. For instance, the periodic exchange of telemetry data between all swarm members provides the foundation for formation flight and collision avoidance. However, due to the mobility of the vehicles and instability of wireless transmissions, maintaining a secure and reliable all-to-all communication remains challenging. This paper investigates encrypted and authenticated multi-hop broadcast communication based on the transmission of custom IEEE 802.11 Wi-Fi data frames.

==> outtakes.tex <==
% middleware
The middle-ware in a drone system must facilitate the efficient movement of information and control signals between different parts of hardware and software. It is crucial to design the system so that the control unit can process information from the sensors on the drone and send commands to the sensors, rotors, and actuators. The control unit makes decisions based on the defined flight mission, the collision avoidance algorithm, and the information from the sensors. Different middle-wares that allow integration of different distribution systems have been proposed to meet the modularity and versatility needs of IoT systems. \cite{Liu2003} implemented a middle-ware called Impala using an asynchronous method for handling requests and responses to achieve a  modular and adaptive solution for WSNs. Impala also provides a way to receive software updates via the node's wireless transceiver and to apply them to the system during run-time. This gives a higher degree of adaptability for long-running autonomous parallel systems. Another work, \cite{Heinzelman2004}, uses a middle-ware they call MiLAN that enables defining different network and sensor management policies based on the application and demonstrates its effectiveness in a sensor-based personal health monitor application. PRISMA in \cite{SilvaJosC3A9} defines a heterogeneous and hierarchical WSN with three levels: (i) Gateway, (ii) Cluster Head, and (iii) Sensor Node. The Gateway level manages the network by making global decisions on the system operation. The Cluster Heads control their respective local clusters in the network. The Cluster Heads themself are Sensor nodes, but they require higher computational power since they should manage the functions of their cluster of sensors. The lowest level contains the ordinary Sensor Nodes that collect environmental information and make local decisions. The middle-ware designer in this method should define the granularity of each level in this hierarchy.

% Just mentioned indirect in the paper, maybe in next session
\cite{Tan2021a} compiles a review of Coverage Path Planning (CPP) in all kinds of autonomous vehicles. The CPP is the determination of the path that covers all points from an initial state to a final state while detecting and avoiding obstacles in a target environment. However, CPP comes with some challenges, one of which is the problem of handling potential uncertainty failures and unknown obstacles in a complex environment. Many of the subcategories of CPP take the environment being obstacle-free as an assumption. Some of the subcategories of CPP have some partial solutions to recalculate the path when encountered with a new obstacle, but they come with other shortcomings, like the inability of the vehicle to escape from the dead zone and the assumption that the new obstacle is a stationary one. Few algorithms like Theta* can handle dynamic obstacles, but they suffer from a high computation time and also neglect the kinematic constraints of the vehicle. \cite{huang_development_2018, faria_applying_2019, faria_efficient_2019, faria_autonomous_2019}

In \cite{Barrientos2011AerialRS} author proposed dividing the coverage area into non-overlapping grid-shape sub-sections and assigning each to one UAV.
In \cite{inbook}, they present a path planning method for a swarm of UAVs to cover irregular-shaped areas. Accordingly, they divide the irregular-shaped areas between UAVs based on each UAV's capabilities, such as the amount of flight time left. They then assign each sub-section to one UAV that executes a zig-zag path pattern according to the shape of the area and characteristics to minimize the number of turns. 

A neural network approach for UAV swarm coverage, where each UAV sees other UAVs as moving obstacles was proposed by \cite{Luo2002ARC}. 
The neural network-based UAV swarm area coverage was inspired by a single UAV neural network area coverage. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Types of Swarm Missions}

% TODO This is an extended copy of the introduction section without any additional insight. We would be better off, deleting this.

% Introduction farming
Many agricultural applications aim at early detection of problems through image-based assessment. Examples include soil analysis, crop health indicators, and growth monitoring. A major challenge is to cover large agricultural areas in acceptable flight time at the required level of detail. Fixed-wing aircraft are a popular solution because of their longer flight time. But they are less agile to control in airspace with adaptive modified trajectories. Consequently, their use is limited to flat terrain with large individual distances. 

% Spot farming
Specialized vehicles enable precision agriculture, for example, to target fertilizers, fungicides and pesticides at the detailed level of individual crops. Via novel approaches to seeding, this enables symbiotic cultivation of multiple compatible crops in locations specifically suited to them. As a result, monocultures are better protected from pests and weather-related unpredictability through complementary plantings. This increases the probability of growth, allows potential crop yield to be estimated more accurately, and supports more sustainable field management. 

% wheat harvesting / animals
This approach is particularly helpful in wheat harvesting for which large combines and tractors with cargo trailers are used. In advance, hidden wild animals such as fawns or wild boar piglets can be protected from the harvesters through targeted detection and eviction. In the future, harvesters will use this data in combination with drone swarms to adjust their harvest routes accordingly.

% Industrial approach bridge inspection
In industrial inspection of complex structures, UAVs can be used in a swarm due to their height, kinetic energy or inaccessible construction. In bridge inspection, the investigation can be done in parallel from different perspectives. Thus, the load-bearing capacity of the structure can be inspected from above, inside and below the structure due to the material properties. Such a three-dimensional modeling of the bridge structure makes it possible to work out the extent of the necessary repair from the data obtained, by embedding the actual condition in risk scenarios. 

% inspection wind turbines
This approach can be adapted to swarm-combined UAVs for the inspection of large wind turbines and rotor blades. These are often standardized models from specialized manufacturers that must be inspected at regular intervals by industrial climbers. To do this, the wind turbines must be shut down periodically to protect the climbers. An adaptive drone swarm can be deployed risk-free from multiple perspectives simultaneously during ongoing operations. By integrating object construction plans, routine inspections can be performed without highly specialized knowledge. By integrating prior experience, vulnerabilities can be examined in greater depth on a regular basis. 

% perimeter protection
Perimeter protection in industrial plants often means controlling fugitive emissions by radio-logical measurements. This presents hurdles for deployed personnel in terms of occupational safety during measurements and the difficulty of accessibility during plant operations. Drones can fly over such areas at a shorter distance from the possible leakage under investigation and collect further information on the presence and extent of fugitive emissions with high data density using specialized sensor technology.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Safety and Security aspects}

% TODO way too generic, no concrete requirements derived

For a successful swarm mission, measures for communication data authenticity, integrity, and confidentiality as well as cyber-attack detection mechanisms need to implemented. For instance, Advanced Encryption Standard (AES) is one of the most common encryption standard, widely supported by the hardware accelerators. Hardware accelerated AES can be used to encrypt critical communication data and prevent information leakage through unauthorized eavesdropping. To ensure that the message is not manipulated along the way by an adversary in a MITM attack, each sent message can be signed using a digital signature to provide the integrity of communication and control commands. Including a timestamp with each sent message can help mitigate replay attacks. Additionally, jamming and spoofing detection mechanisms can provide an additional level of security by detecting adversaries in early phases and thus, preventing the consequences of cyber-attacks. 

Another part of UAV security and safety are the fail-safe mechanisms. Fail-safe mechanisms ensure that in case of a communication signal loss, low battery, or other unexpected system failures, the UAV can still safely land or return to the launch position without causing a crash. Only collective implementation of the above mentioned security and safety mechanisms can ensure the safe operation and mission success.


% TODO we don't need formation flight outside of the intruction. We do not work on formation flight. Oscar focuses on collision avoidance by force-field based path planning. Here we need just the rough idea, pointing out that the same data as in the previous subsection is needed but allows to fly around obstacles instead of just slowing down and stopping.

In formation flight, a group of drones work together to achieve a common goal by coordinating their movements in a specific formation. This approach is based on the principles of swarm robotics to use multiple autonomous agents to perform a task more efficiently and effectively than a single agent. Formation flight in a drone swarm has several benefits, such as increased coverage area, enhanced situational awareness, and improved fault tolerance.

Formation flight can be helpful in the path planning for drone swarm missions. It can enable the swarm drones to cover a larger area and gather more data or perform more tasks than they would individually. Formation flight can also help these drones optimize their trajectories and avoid collisions with each other and obstacles in the environment. By exchanging information and adapting to changes in mission requirements, swarm drones can work together more effectively and achieve their objectives more efficiently. Overall, formation flight in a drone swarm can be a powerful tool for improving the performance and capabilities of autonomous systems. It also enables the drones to find their path after a change in their original path due to collision avoidance.
